3D hydrodynamic simulations of massive main-sequence stars II. Convective excitation and spectra of internal gravity waves

Recent photometric observations of massive stars have identified a low-frequency power excess which appears as stochastic low-frequency variability in light curve observations. We present the oscillation properties of high resolution hydrodynamic simulations of a 25 $\mathrm{M}_\odot$ star performed with the PPMStar code. The model star has a convective core mass of $\approx\, 12\, \mathrm{M}_\odot$ and approximately half of the envelope simulated. From this simulation, we extract light curves from several directions, average them over each hemisphere, and process them as if they were real photometric observations. We show how core convection excites waves with a similar frequency as the convective time scale in addition to significant power across a forest of low and high angular degree $l$ modes. We find that the coherence of these modes is relatively low as a result of their stochastic excitation by core convection, with lifetimes on the order of 10s of days. Thanks to the still significant power at higher $l$ and this relatively low coherence, we find that integrating over a hemisphere produces a power spectrum that still contains measurable power up to the Brunt--V\"ais\"al\"a frequency. These power spectra extracted from the stable envelope are qualitatively similar to observations, with same order of magnitude yet lower characteristic frequency. This work further shows the potential of long-duration, high-resolution hydrodynamic simulations for connecting asteroseismic observations to the structure and dynamics of core convection and the convective boundary.

==> paper_resources/macros/vectors.tex <==
%=======================================================================
%
% vectors.tex---some basic vector operators
%
% Requires package bm.sty
%
%=======================================================================

\RequirePackage{bm}
%\RequirePackage{amssymb}
%\RequirePackage{amsbsy}
\newcommand{\bvec}[1]{\ensuremath{\boldsymbol{#1}}} %boldface vector style
\newcommand{\grad}{\bvec{\nabla}} %gradient
\newcommand{\divr}{\nabla \cdot} %divergence
\newcommand{\curl}{\bvec{\nabla \times}} %curl
\newcommand{\lap}{\ensuremath{\nabla^2}} %Laplacian
\newcommand{\btens}[1]{\ensuremath{\boldsymbol{\mathsf{#1}}}}
\newcommand{\vcross}{\bvec{\times}}
\newcommand{\vdot}{\bvec{\cdot}}
% end vectors.tex

